On the Effectiveness of Equivariant Regularization for Robust Online Continual Learning

Humans can learn incrementally, whereas neural networks forget previously acquired information catastrophically. Continual Learning (CL) approaches seek to bridge this gap by facilitating the transfer of knowledge to both previous tasks (backward transfer) and future ones (forward transfer) during training. Recent research has shown that self-supervision can produce versatile models that can generalize well to diverse downstream tasks. However, contrastive self-supervised learning (CSSL), a popular self-supervision technique, has limited effectiveness in online CL (OCL). OCL only permits one iteration of the input dataset, and CSSL's low sample efficiency hinders its use on the input data-stream. In this work, we propose Continual Learning via Equivariant Regularization (CLER), an OCL approach that leverages equivariant tasks for self-supervision, avoiding CSSL's limitations. Our method represents the first attempt at combining equivariant knowledge with CL and can be easily integrated with existing OCL methods. Extensive ablations shed light on how equivariant pretext tasks affect the network's information flow and its impact on CL dynamics.

==> content/tables/abl_mcd.tex <==
\rowcolors{2}{lightgray}{}
\begin{tabular}{lcc}
\toprule
\textbf{AUROC \%} & \textbf{ER-ACE}~\cite{caccia2022new} & \textbf{X-DER}~\cite{boschini2022class}\\
\midrule
Baseline & $68.60$ & $72.34$ \\
~+~\methnam & $71.48$\errino\underline{\gainped{2.88}} & $75.53$\errino\underline{\gainped{3.19}} \\
~+~CSSL & $70.75$\gainped{2.15} & $72.43$\gainped{0.09}\\
\bottomrule
\end{tabular}
\vspace{1em}


==> content/tables/acc_bothil.tex <==
\begin{table*}[t] % MIXED TABLE
    \centering
    % \resizebox{\textwidth}{!}{
    \rowcolors{2}{}{lightgray}
    \setlength{\tabcolsep}{2.4pt}
    
    \begin{tabular}{lcccc|cccc}
    \toprule
    & \multicolumn{4}{c}{\textbf{\classil}} & \multicolumn{4}{c}{\textbf{\taskil}} \\
    Method & \multicolumn{2}{c}{\textbf{Seq.\ CIFAR-100}} & \multicolumn{2}{c}{\textbf{Seq.\ \miniimagenet}} & \multicolumn{2}{c}{\textbf{Seq.\ CIFAR-100}} & \multicolumn{2}{c}{\textbf{Seq.\ \miniimagenet}} \\
    \midrule    
    Joint-offline & \multicolumn{2}{c}{\result{69.47}{0.20}{-}}                    & \multicolumn{2}{c}{\result{63.31}{0.47}{-}} & \multicolumn{2}{c}{\result{82.69}{0.31}{-}}        & \multicolumn{2}{c}{\result{87.55}{0.16}{-}}  \\
    Joint-online & \multicolumn{2}{c}{\result{23.14}{0.74}{-}}                    & \multicolumn{2}{c}{\result{10.68}{0.67}{-}} & \multicolumn{2}{c}{\result{54.12}{1.45}{-}}        & \multicolumn{2}{c}{\result{52.62}{0.98}{-}}         \\
    Finetune        & \multicolumn{2}{c}{\result{7.00}{0.15}{100}}    & \multicolumn{2}{c}{\result{3.21}{0.10}{100}}          & \multicolumn{2}{c}{\result{35.42}{3.11}{44.32}}    & \multicolumn{2}{c}{\result{31.55}{2.64}{28.75}}     \\
    \midrule
\rowcolor{white}\textbf{Buffer Size} & 500 & 2000 & 2000 & 8000 & 500 & 2000 & 2000 & 8000 \\
    \midrule
    ER-ACE~\cite{caccia2022new}      & \result{20.17}{1.31}{38.75} & \result{26.95}{1.12}{23.69} & \result{15.03}{0.63}{35.01} & \result{16.07}{1.29}{37.94} & \result{56.06}{1.41}{9.48} & \result{64.94}{1.11}{3.19} & \result{64.68}{1.21}{\underline{3.77}} & \result{66.17}{1.96}{\underline{4.10}} \\
    ~+~\methnam & \resultj{\textbf{24.01}}{1.43}{\underline{35.88}} & \resultj{\textbf{31.07}}{1.53}{\underline{20.36}} & \resultr{\textbf{18.08}}{1.46}{\underline{32.53}} & \resultj{\textbf{18.43}}{0.95}{\underline{33.22}} & \resultj{\textbf{61.35}}{1.28}{\underline{9.23}} & \resultj{\textbf{69.41}}{1.64}{\underline{2.89}} & \resultr{\textbf{68.02}}{1.32}{5.27} & \resultj{\textbf{69.13}}{1.42}{4.11} \\
    X-DER~\cite{boschini2022class}   & \result{25.80}{0.98}{39.54} & \result{30.44}{0.80}{31.52} & \result{17.51}{1.08}{34.25} & \result{18.01}{1.54}{50.84} & \result{63.10}{0.86}{4.31} & \result{69.00}{0.83}{1.38} & \result{67.67}{1.19}{4.71} & \result{68.97}{1.32}{4.39} \\
    ~+~\methnam & \resultj{\textbf{29.35}}{0.72}{\underline{35.56}} & \resultj{\textbf{34.57}}{0.96}{\underline{29.71}} & \resultj{\textbf{21.26}}{0.91}{\underline{34.07}} & \resultj{\textbf{21.71}}{1.30}{\underline{34.76}} & \resultj{\textbf{68.19}}{1.08}{\underline{2.98}} & \resultj{\textbf{73.45}}{0.55}{\underline{0.97}} & \resultj{\textbf{71.32}}{0.86}{\underline{3.01}} & \resultj{\textbf{72.39}}{0.89}{\underline{2.66}} \\
    CoPE~\cite{de2021continual}      & \result{19.98}{1.49}{75.32} & \result{34.09}{2.12}{46.39} & \result{22.67}{1.32}{57.96} & \result{24.54}{2.67}{55.09} & \result{51.89}{1.64}{23.46} & \result{66.56}{2.13}{7.48} & \result{70.10}{1.42}{\underline{4.89}} & \result{73.61}{2.36}{3.58} \\
    ~+~\methnam & \resultj{\textbf{26.15}}{1.16}{\underline{69.28}} & \resultj{\textbf{38.48}}{1.48}{\underline{45.50}} & \resultr{\textbf{25.91}}{1.67}{\underline{57.73}} & \resultr{\textbf{26.76}}{1.17}{\underline{52.69}} & \resultj{\textbf{60.19}}{1.23}{\underline{20.34}} & \resultj{\textbf{71.91}}{0.90}{\underline{6.42}} & \resultr{\textbf{71.17}}{1.05}{5.30} & \resultr{\textbf{75.33}}{1.27}{\underline{2.54}} \\
    \midrule
    DualNet~\cite{pham2021dualnet}   & \result{11.09}{0.51}{92.42} & \result{19.93}{0.74}{73.44} & \result{16.21}{1.13}{80.35} & \result{25.33}{1.47}{59.60} & \result{49.38}{0.65}{25.20} & \result{57.05}{0.63}{13.85} & \result{68.43}{0.46}{9.99} & \result{73.89}{0.99}{5.54} \\
    ~+~\methnam & \resultr{\textbf{11.89}}{0.61}{\underline{89.97}} & \resultj{\textbf{20.88}}{0.90}{\underline{73.02}} & \resultr{\textbf{18.66}}{1.00}{\underline{72.74}} & \resultr{\textbf{30.90}}{0.86}{\underline{52.14}} & \resultr{\textbf{50.11}}{0.69}{\underline{23.94}} & \resultj{\textbf{59.66}}{0.39}{\underline{12.99}} & \resultr{\textbf{70.26}}{0.84}{\underline{7.39}} & \resultr{\textbf{76.97}}{0.33}{\underline{3.87}} \\
    \bottomrule
    \end{tabular}
    % }
    \caption{Final Average Accuracy $\bar{A}_F$ ($\uparrow$) and Final Average Adjusted Forgetting ($\bar{F}^*_F$) ($\downarrow$) on the \classil setting. \errino indicates a result obtained with rotation, \jayino a result obatined with $2\times2$ jigsaw puzzle.}
    \label{tab:cil_main}
\end{table*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
